Unlocking the Power of Environment Assumptions for Unit Proofs

Clearly articulating the assumptions of the execution environment is crucial for the successful application of code-level formal verification. The process of specifying a model for the environment can be both laborious and error-prone, often requiring domain experts. In contrast, when engineers write unit tests, they frequently employ mocks (tMocks) to define the expected behavior of the environment in which the function under test operates. These tMocks describe how the environment behaves, e.g., the return types of an external API call (stateless behaviour) or the correct sequence of function calls (stateful behaviour). Mocking frameworks have proven to be highly effective tools for crafting unit tests. In our work, we draw inspiration from tMocks and introduce their counterpart in the realm of formal verification, which we term vMocks. vMocks offer an intuitive framework for specifying a plausible environment when conducting code-level formal verification. We implement a vMock library for the verification of C programs called SEAMOCK. We investigate the practicality of vMocks by, first, comparing specifications styles in the communication layer of the Android Trusty Trusted Execution Environment (TEE) open source project, and second, in the verification of mbedTLS, a widely used open source C library that provides secure communication protocols and cryptography primitives for embedded systems. Based on our experience, we conclude that vMocks complement other forms of environment models. We believe that vMocks ease adoption of code-level formal verification among developers already familiar with tMocks.

==> intro.old.tex <==
\section{Introduction}

% \seamock transforms DSL expectations into environment functions during compilations, thereby minimizing verification overhead.

% Similar to tMocks, a vMocks captures the anticipated behaviors of the environment when invoked by a program function. During verification, the vMock reproduces these anticipated behaviors. To define these behaviors, vMocks employ a tMock-like Domain-Specific Language (DSL), enabling users to articulate only the essential expectations.


% To make software verification manageable,
% every software verification effort chooses a system boundary of what is of interest and what is considered outside scope.
% This boundary conceptually creates a system under test (\sut) and the rest of the codebase -- called the \textit{Environment}.
% The \env is operationally a set of function calls that provide valid data to the \sut.
% There are various design choices available on how to model the environment.
% An \env can be stateless --- returning fresh non deterministic values on each function call.
% Alternatively, it can be stateful.
% This state embodies a stronger specification of the environment needed for the correct operation of the \sut.
% If a stateless \env is adequate, each function call can be modelled using a \textit{function summary}.
% Function summaries are declarative specifications that assume a simple \env without any state.
% If the \env needs to have state then it can be modelled using a \textit{fake}\footnote{Fakes are also called stubs, but we prefer the GoogleTest terminology.}.
% Writing and tuning a useful environment model for verifying an industrial codebase may take months to years~\cite{DBLP:conf/fmcad/LahiriLGNLKDLB20,DBLP:conf/eurosys/BallBCLLMORU06}.
% We present \textit{vMocks} as a way to reduce the burden for specifying environments used in verification, inspired by their use in testing (tMocks)~\cite{DBLP:conf/oopsla/FreemanMPW04a}.


To facilitate software verification, each verification task defines a system boundary, which delineates what is within the scope of interest and what lies outside of it. This boundary essentially creates two key components: the System Under Verification (\sut\footnote{We use SUT as an acronym instead of SUV since it is more familiar.}) and the \env, which encompasses the rest of the system. The environment, operationally, is a series of function calls that supply valid data to the \sut.
When it comes to modeling the \env, there are several design choices at hand. The \env can either be stateless, where it provides fresh, non-deterministic values with each function call, or stateful, in which case it holds a more comprehensive specification of the environment required for the SUT to function correctly. In the case of a stateless environment, each function call can be represented using a function summary, which is a declarative specification assuming a simple stateless environment.
However, if the environment requires state, it can be modeled using a construct referred to as a \emph{fake}. It's worth noting that creating and fine-tuning an effective environment model for the verification of a complex industrial codebase is a time-consuming process, often taking months to years~\cite{DBLP:conf/fmcad/LahiriLGNLKDLB20,DBLP:conf/eurosys/BallBCLLMORU06}.

In this article, we introduce vMocks as a solution aimed at alleviating the challenge of specifying environments for the purpose of verification. vMocks draw inspiration from their counterparts used in testing, known as tMocks~\cite{DBLP:conf/oopsla/FreemanMPW04a}. Similar to a tMock, a vMock captures the anticipated behavior of the environment when invoked by a program function. During verification, the vMock reproduces these anticipated behaviors. To define these behaviors, vMocks employ a tMock-like Domain-Specific Language (DSL), enabling users to articulate only the essential expectations.
\newsavebox{\figturtle}%
\begin{lrbox}{\figturtle}%
\begin{lstlisting}[basicstyle=\footnotesize, language=C++, escapechar=@, numbers=left]
class Turtle {
  ...
  virtual ~Turtle() = default;
  void PenUp() {...}
  virtual void PenDown() = 0;
};
\end{lstlisting}%
\end{lrbox}%

\newsavebox{\figmockturtle}%
\begin{lrbox}{\figmockturtle}%
\begin{lstlisting}[basicstyle=\footnotesize, language=C++, escapechar=@, numbers=left]
#include "turtle.h"       // Brings in Turtle class
#include "gmock/gmock.h"  // Brings in gMock.
#include "gtest/gtest.h"

class MockTurtle : public Turtle {@\label{line:gmock_turtle_mock_class}@
 public:
  ...
  MOCK_METHOD(void, PenDown, (), (override));
};
using ::testing::AtLeast;

TEST(PainterTest, CanDrawSomething) {
  MockTurtle turtle;
  EXPECT_CALL(turtle, PenDown()).Times(AtLeast(1));@\label{line:gmock_turtle_expect}@
  Painter painter(&turtle);
  EXPECT_TRUE(painter.DrawCircle(0, 0, 10));
}
\end{lstlisting}%
\end{lrbox}%

\begin{figure}[t]
\centering
\begin{subfigure}{0.4\textwidth}
\scalebox{0.8}{\usebox{\figturtle}}
\caption{Class to be mocked.}
\label{fig:turtle_gmock_example}
\end{subfigure}%
\quad
\begin{subfigure}{0.4\textwidth}
\scalebox{0.8}{\usebox{\figmockturtle}}
\caption{A gMock usage example.}
\label{fig:gmock_example}
\end{subfigure}
\caption{An adaptation from GoogleTest documentation.}
\end{figure}%
% In test driven development (TDD), tMocks are used extensively to specify behavior of dependencies one does not wish to test, i.e., the environment.
% We motivate this discussion by adapting an example from the documentation of gMock\footnote{GoogleMock is abbreviated to gMock for brevity.}~\cite{GoogleTest} -- a popular open source mocking framework for C++.
% ~\cref{fig:turtle_gmock_example} shows a \code{Turtle} class that is the environment we want to test against.
% The \sut is the \code{Painter} class and the function to be unit tested is~\code{Painter::DrawCircle}, which needs  the \code{Turtle} environment.
% The unit test is shown in~\cref{fig:gmock_example}.
% We create a mock \code{Turtle} environment at~\lref{line:gmock_turtle_mock_class}.
% The methods to be mocked are defined using \code{MOCK_METHOD}.
% Moving to the actual unit test \code{CanDrawSomething}, a behavior expectation on the mock turtle is defined at~\lref{line:gmock_turtle_expect}.
% We expect that the subsequent \code{painter.DrawCircle} call will invoke the \code{Turtle::PenDown} method atleast once.
% If this expectation is not met then the test fails.
\sid{move up}
Mocking frameworks, such as GoogleMock~\cite{GoogleTest} (or gMock for short), are used extensively in unit testing. They enable developers to specify behavior of the environment of the function under test.  

For example, ~\cref{fig:turtle_gmock_example} shows a \code{Turtle} class that is the environment we want to test against.
The \sut is the \code{Painter} class. The function to be unit tested is~\code{Painter::DrawCircle}, which needs  the \code{Turtle} environment.
The unit test is shown in~\cref{fig:gmock_example}.
We create a mock \code{Turtle} environment at~\lref{line:gmock_turtle_mock_class}.
The methods to be mocked are defined using \code{MOCK_METHOD}.
Moving to the actual unit test \code{CanDrawSomething}, a behavior expectation on the mock turtle is defined at~\lref{line:gmock_turtle_expect}.
We expect that the subsequent \code{painter.DrawCircle} call will invoke the \code{Turtle::PenDown} method at least once.
If this expectation is not met then the test fails. 

We make two key observations. First, the tMock is partial, i.e., it need not define all methods of a class. For example, \code{PenUp} is not mocked since we never expect it to be called in the unit test.
Second, tMocks specify how the environment is to behave with external observers; this differentiates a tMock and, what is known in testing as, a fake environment. \sid{move up} A \fak environment is simpler than an actual environment.
However, it is still an operational model.
As an example when one creates a file system \fak, it is a collection of file-like objects, albeit in-memory instead of on-disk.
\otoh, a mock only specifies how the environment behaves when it is interacted with in some specific way.
Thus, a tMock file system can be specified to return a particular value the first time it is called, and throw an exception if called again.
This specification style makes mocks well suited for unit testing, where the focus is on how a function behaves in isolation given behavioral specifications of the environment, rather than the how the \sut interacts with the environment as a whole.

We believe the application of mocks to code-level formal verification has two benefits.
First, it lowers the barrier for starting on formal verification by building on developer's experience in mocking for testing.
Second, verifying functions at a unit level facilitates early formal verification of the \sut, again, by the same developers writing production code before changes are submitted.
This is in contrast to waiting for the \sut to be sufficiently developed and only then developing the necessary, possibly \fak, environment for formal verification.

Though handy, vMocks are not a substitute for \faks.
Fakes are better for integration proofs -- symbolic tests that verify code flow across multiple functions. These tests usually require stateful \envs and mocks become brittle and cumbersome to write and maintain with these requirements.

% \bparagraph{Goals.}
\sid{modified!}
% Both function summaries and fakes are useful in building confidence in software. We do not aim to replace either with vMocks.Instead
% This paper studies the idea of using environment models specified as mocks to enable development and verification in lockstep, i.e, verification driven development.
% First, we explore an application of vMocks to development of unit proofs\footnote{A unit proof is analogous to a unit test, but for verification} that are executable in \seabmc, the bounded model checking engine for \seahorn~\cite{DBLP:conf/fmcad/PriyaSBZVG22}.
% Second, we describe \seamock -- a verification oriented DSL implementation inspired by \gmock.
% The \seamock library is open-sourced. \sid{redacted url} %at \url{https://github.com/seahorn/seamock}.
% \cmock provides a language for specifying mocks similar to \gmock.
% The novelty of \cmock is that these specifications are preprocessed to ordinary C functions at compile time unlike \gmock where runtime polymorphism is used in constructing mocks.
% We posit that the zero-cost abstraction of \cmock is advantageous for static analysis tools since the generated code contains less indirection (e.g., vtables, function pointers) overall and, thus, is easier to reason with in a static setting.
% Third, we evaluate rapid verification of 6000 lines of industrial code using \seamock.
% \sid{make it stronger!}In summary, mock environments can be useful in formally verifying properties of a \sut and complement other ways of specifying environments.

\ag{The contribution of SeaMock as a library is mixed together with everything else. Pull it out into a seaprate paragraph. First explain why we do not want to use existing mocking libraries. Then explain seamock.}

\ag{Conclude with a tight paragraph of contributions. The intro is pretty long and the core contributions are lost.}

This paper proposes a mocking framework for modelling assumptions of environment for code-level verification. First, we describe an application of vMocks in the development of unit proof harness\footnote{A unit proof is analogous to a unit test, but for verification.} that are executable in \seabmc, the bounded model checking engine for \seahorn~\cite{DBLP:conf/fmcad/PriyaSBZVG22}.
Second, we describe \seamock -- a verification oriented DSL implementation inspired by \gmock.
The \seamock library is open-sourced\footnote{URLs to code repositories will be added in the final version.}. \sid{redacted url} %at \url{https://github.com/seahorn/seamock}.
\cmock provides a language for specifying mocks similar to \gmock.
The novelty of \cmock is that these specifications are pre-processed to ordinary C functions at compile time unlike \gmock where runtime polymorphism is used in constructing mocks.
We posit that the zero-cost abstraction of \cmock is advantageous for static analysis tools since the generated code contains less indirection (e.g., vtables, function pointers) overall and, thus, is easier to reason with in a static setting.
Finally, we evaluate the practicality and effectiveness of vMocks by employing them in the context of the verification of two open-source libraries: 
  \begin{inparaenum}[(1)]
  \item the communication layer in the Android Trusty trusted execution environment (TEE) and
  \item mbedTLS~\cite{mbedTLS}, a widely used C library that implements secure communication protocols and cryptography primitives suitable for embedded systems. 
  \end{inparaenum}
  Based on our experiences, we find that vMocks complement other forms of environment models. We believe that vMocks will enable the early adoption of code-level formal verification among developers already familiar with tMocks.
\sid{add more background about solution}

The rest of the paper is organized as follows: .

In \cref{sec:motivation}, we motivate vMocks by exploring the use of fakes, summaries, and mocks for verification of small module in TEE. In \cref{sec:seamock}, we present the design and implementation of \seamock library. In \cref{sec:evaluation}, we describe an extensive evaluation of vMocks on verification of memory safety of \mbedtls. We discuss usability issues in \cref{sec:use}, related work in \cref{sec:related}, and conclude in \cref{sec:conclusion}.

==> todos.tex <==
\section{TODOS}

\bparagraph{Known issues}
  \begin{todolist}
  \end{todolist}

